Asymptotically Optimal Sampling-based Kinodynamic Planning

Sampling-based algorithms are viewed as practical solutions for high-dimensional motion planning. Recent progress has taken advantage of random geometric graph theory to show how asymptotic optimality can also be achieved with these methods. Achieving this desirable property for systems with dynamics requires solving a two-point boundary value problem (BVP) in the state space of the underlying dynamical system. It is difficult, however, if not impractical, to generate a BVP solver for a variety of important dynamical models of robots or physically simulated ones. Thus, an open challenge was whether it was even possible to achieve optimality guarantees when planning for systems without access to a BVP solver. This work resolves the above question and describes how to achieve asymptotic optimality for kinodynamic planning using incremental sampling-based planners by introducing a new rigorous framework. Two new methods, Stable Sparse-RRT (SST) and SST*, result from this analysis, which are asymptotically near-optimal and optimal, respectively. The techniques are shown to converge fast to high-quality paths, while they maintain only a sparse set of samples, which makes them computationally efficient. The good performance of the planners is confirmed by experimental results using dynamical systems benchmarks, as well as physically simulated robots.

==> lemma_close_exist.tex <==
\begin{lemmma}
 Let there be a trajectory $\pi$ satisfying
 Eq. \ref{eq:dynamics}. Then there exists a positive value $\delta_0$,
 such that: $\forall\ \delta \in (0,\delta_0]$, $\forall\
 x_{0}^\prime\in\ball_\delta(\pi(0))$, and $\forall\
 x_{1}^\prime\in\ball_\delta(\pi(t))$, there exists a trajectory
 $\pi^\prime$, so that: (i) $\pi^\prime(0)=x_{0}^\prime$ and
 $\pi^\prime(t^\prime)=x_1^\prime$; (ii) $\pi$ and $\pi^{\prime}$ are
 $\delta$-similar trajectories.
\label{lem:closeexist}
\end{lemmma}

%%%%%%%%%%%%%%%%%%%% add a heuristic proof %%%%%%%%%%%%%%%%%%%%%%%%%

Informally speaking, \emph{Chow's} condition (assumption \ref{ass:system}) implies 
that \emph{Ball Box} theorem holds. It also implies that the manifold $\Xfree$ is 
\emph{regular} and \emph{involutory}\cite{Choset2005Principles-of-R}.
In the case of real-analytic control-affine system, it is \emph{STLA}, if 
and only if the \emph{distribution} satisfies \emph{Chow's} condition\cite{Sussmann-LocalControllability1987}. 
Assume every state on the optimal trajectory is a \emph{regular point}. Then,
the \emph{sub-Riemannian ball} up to a small constant radius $t_\epsilon$ 
contains a weighted box of the same dimension of the state space and it is 
oriented according to vector fields of the \emph{Lie brackets}. The bases are real 
analytical. Therefore there exists a open neighborhood of each point $x$ such that the
bases evaluated at a different point $x^\prime$ converge to the bases at $x$ as $x^\prime\to x$.
Then, the weighted boxes centered by two sufficiently 
close states has non-empty intersection. It implies that a hyper ball of some 
positive radius $\delta_0$ can be fitted into this intersection region. In sum, there exists two 
sufficiently close hyper ball regions on the optimal trajectory such that between any point $x$ in one 
ball and any point in the other ball there exists a horizontal curve and the length of the curve is 
less or equals to the radius $t_\epsilon$ of the \emph{sub-Riemannian ball}. Then concatenating all 
hyper balls, for the optimal trajectory, there exists $\delta$-similar trajectories. From a different 
perspective, Lemma \ref{lem:closeexist} is a necessary condition for all systems 
where \rrtstar\ converges.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> theorem_bn_finite.tex <==
\begin{thm}
For a $\delta$-robust optimal trajectory consisting of $k>0$ segments, and a fixed $\rho_{\delta\to\delta_{BN}} > 0$, the iterations $N_{\rho_{\delta\to\delta_{BN}}}$ for the algorithm to generate a near-optimal solution with probability greater than $1-e^{-1}$ can be bounded by:
$\frac{1}{1-e^{-1}}\cdot\frac{k}{\gamma\rho_{\delta\to\delta_{BN}}}$
\label{thm:convergenRateBN}
\end{thm}
% \vspace{-.2in}

The above theorem argues that in order to achieve at least $1-e^{-1}\approx 63.21\%$ probability for \rrtbestnear\ to generate 
a near-optimal trajectory, the needed iterations can be upper bounded. This bound is in the same order as the expected 
number of iterations for \rrt\ to return a solution \cite{LaValle2001}. 

%%%%%%%%%%%%%%%%%%%%%% begin proof for convergence rate %%%%%%%%%%%%%%%%%%%%%%%%
{\bf Proof:} Firstly, consider $B_{\delta_{BN}}(x_1^\ast)$, and from \edited{Equation} (\ref{eq:Epropagate}), 
\vspace{-.1in}
\begin{align*}
\Prob(E_1^{(n)})	&\geq 1-\prod_{i=1}^n(1-\gamma\rho_{\delta\to\delta_{BN}})\\
				&=1-(1-\gamma\rho_{\delta\to\delta_{BN}})^n\\
				&= 1-(1-\gamma\rho_{\delta\to\delta_{BN}})^{\frac{1}{\gamma\rho_{\delta\to\delta_{BN}}}\gamma\rho_{\delta\to\delta_{BN}}n}\\
				&> 1-(e^{-1})^{\gamma\rho_{\delta\to\delta_{BN}}n}
\end{align*}

\noindent
Clearly, if $n\geq\frac{1}{\gamma\rho_{\delta\to\delta_{BN}}}$, then $\Prob(E_1^{(n)})>1-e^{-1}$.

\noindent
Next, consider $B_{\delta_{BN}}(x_{k+1}^\ast)$, and use $\Prob(E_k^{(n)})>1-e^{-1}$ as the induction assumption, from \edited{Equation} (\ref{eq:Epropagate}),
\vspace{-.1in}
\begin{align*}
\Prob(E_{k+1}^{(n)}) &\geq 1-\prod_{i=1}^n(1-\gamma\rho_{\delta\to\delta_{BN}}\Prob(E_k^{(i)}))\\
				&> 1-\prod_{i=1}^n(1-\gamma\rho_{\delta\to\delta_{BN}}(1-e^{-1}))\\
				&= 1-(1-\gamma\rho_{\delta\to\delta_{BN}}(1-e^{-1}))^n
\end{align*}
\noindent
Similar to the reasoning for $\Prob(E_1^{(n)})$, if $\Delta n\geq\frac{1}{\gamma\rho_{\delta\to\delta_{BN}}(1-e^{-1})}$, then $\Prob(E_{k+1}^{(n)})>1-e^{-1}$, where $\Delta n=n-\frac{1}{\gamma\rho_{\delta\to\delta_{BN}}}$.
\noindent
Inductively, there is, if $n\geq\frac{k+1}{\gamma\rho_{\delta\to\delta_{BN}}(1-e^{-1})}$, then $\Prob(E_{k+1}^{(n)})>1-e^{-1}$.
\telos

==> theorem_gamma_ratio.tex <==
% \begin{lemmma}
% Given $\delta>0$, and $\delta_{BN}>0$, for a scale $\alpha\in (0,1)$, let $\delta^\prime=\alpha\delta$ and $\delta_{BN}^\prime=\alpha\delta_{BN}$, there is
% \[\frac{\gamma^\prime}{\gamma}=\alpha^d\]
% \label{lem:gammaRatio}
% \end{lemmma}

{\bf Lemma \ref{lem:gammaRatio} }\emph{
Given $\delta>0$, and $\delta_{BN}>0$, for a scale $\alpha\in (0,1)$, let $\delta^\prime=\alpha\delta$ and $\delta_{BN}^\prime=\alpha\delta_{BN}$, there is
\[\frac{\gamma^\prime}{\gamma}=\alpha^d\]
}

{\bf Proof:} Recall that\[\gamma = \frac{ \mu( \{x_{rand}| x_{rand} \in \ball_{x_i,\theta} \cap
  \ball_{x^\prime,\Dnear} \} )} {\mu(\Xfree)}\]

Clearly $\gamma$ is a geometric region in $\Xfree$ where the dimension is $d$. It follows geometric scaling rule.
\telos

==> theorem_rt_sublinear.tex <==
\begin{thm}
For the worst case, the $k^{th}$ segments of the trajectory returned by \rt\ converges sub-linearly to the near optimal solution. e.g.,
\[\lim_{n\to\infty}\frac{|\Prob(E_{k}^{(n+1)}) - 1|}{|\Prob(E_k^{(n)}) - 1|}=1\]
\label{thm:convergenRateRTsublinear}
\end{thm}

{\bf Proof:}
Applying the boundary condition of \edited{Theorem} \ref{eq:Epropagate}, the worst case scenario is that only one state is considered to exist inside each ball region (even there could be multiply states). Without any other system properties, this is the only available information. Then consider the ratio of the probabilities between iteration $k+1$ and $k$.

\begin{align}
\frac{|\Prob(E_{k}^{(n+1)}) - 1|}{|\Prob(E_k^{(n)}) - 1|}
&=\frac{\prod_{j=1}^{n+1}(1-\frac{\Prob(E_{k-1}^{(j)})\cdot\rho}{j})}{\prod_{j=1}^{n}(1-\frac{\Prob(E_{k-1}^{(j)})\cdot\rho}{j})}\notag\\
&=1-\frac{\Prob(E_{k-1}^{(n+1)})\cdot\rho}{n+1}\notag
\end{align}

\noindent Clearly, $\Prob(E_{k-1}^{(n)})$ is at most 1 and $\rho$ is less than 1. Then,
\begin{align}
\lim_{n\to\infty}\frac{|\Prob(E_{k}^{(n+1)}) - 1|}{|\Prob(E_k^{(n)}) - 1|}=\lim_{n\to\infty}1-\frac{\Prob(E_{k-1}^{(n+1)})\cdot\rho}{n+1}=1\notag
\end{align}
\telos

==> theorem_sst_finite.tex <==
\begin{thm}
For a $\delta$-robust optimal trajectory consisting of $k>0$ segments, and a fixed $\rho_{\delta\to\delta_c} > 0$, the iterations $N_{\rho_{\delta\to\delta_c}}$ for the algorithm to generate a near-optimal solution with probability greater than $1-e^{-1}$ can be bounded by:
$\frac{1}{1-e^{-1}}\cdot\frac{k}{\gamma\rho_{\delta\to\delta_c}}$
\label{thm:convergenRateSST}
\end{thm}

==> theorem_sststar_finite.tex <==
\begin{coro}
For small $k_0$, to almost surely return a near-optimal trajectory by Alg. \ref{alg:SSTstar} only happens at time infinity. e.g., $\liminf_{j\to\infty} \mathbb{P}(E_{k,j}) = 1$. If $k_0$ is chosen sufficiently large, Alg. \ref{alg:SSTstar} has guarantee to return a near-optimal trajectory in sufficiently large finite time. e.g., $\mathbb{P}\Big(\liminf_{j\to\infty}E_{k,j}\Big)=1$.
\label{coro:zeta}
\end{coro}

{\bf Proof:}
Let $\neg E_{k,j}$ be the negation of $E_{k,j}$. Then since Eq. \ref{eq:Esimplified}, there is,
\begin{align}
\Prob(\neg E_{k,j}) &< 1 - 1 + P_c (e^{-p_c})^{\beta\cdot(1+\log j)-\gamma^{(j)}\rho^{(j)}c}\notag\\
					&=P_c\cdot (e^{-p_c\beta}) \cdot (e^{-p_c\beta\log j}) \cdot (e^{-p_cc\gamma^{(j)}\rho^{(j)}})
					\label{eq:notErefact}
\end{align}

Clearly, $p_c\cdot c>0$, so $0<e^{-p_cc}<1$. And $\gamma^{(j)}\rho^{(j)}\to 0$ as $j\to\infty$. Therefore for the third term in Eq. \ref{eq:notErefact}, there is $(e^{-p_cc\gamma^{(j)}\rho^{(j)}})<1$. Eq. \ref{eq:notErefact} becomes the following,
\begin{align*}
\Prob(\neg E_{k,j}) < P_c\cdot (e^{-p_c\beta}) \cdot (e^{-p_c\beta\log j})
\end{align*}

To sum up the probabilities of $j$ from $1\to\infty$, there is 
\begin{align}
\sum_{j=1}^\infty \Prob(\neg E_{k,j}) 	&< P_c\cdot (e^{-p_c\beta})\sum_{j=1}^\infty (e^{-p_c\beta\log j})\notag\\
										&= P_c\cdot (e^{-p_c\beta})\sum_{j=1}^\infty \frac{1}{(e^{\log j})^{p_c\beta}}\notag\\
										&= P_c\cdot (e^{-p_c\beta})\sum_{j=1}^\infty \frac{1}{(j)^{p_c\beta}}
										\label{zeta}
\end{align}

Clearly when $p_c\cdot\beta>1$ Eq. \ref{zeta} is \emph{Riemann zeta} function times a constant. It converges when the real part $p_c\cdot\beta>1$ and diverges otherwise. Recall that $\beta=k_0\gamma^{(0)}\rho^{(0)}$, since $\gamma^{(0)}\rho^{(0)}$ is unknown, $p_c\cdot\beta$ is unknown. 

Therefore, when $k_0$ is chosen sufficiently large, Eq. \ref{zeta} converges ($\sum_{j=1}^\infty \Prob(\neg E_{k,j})<\infty$). According to \emph{Borel}-\emph{Cantelli} \emph{lemma}, there is \[\Prob\Big(\limsup_{j\to\infty} \neg E_{k,j}\Big) = 0 \iff \Prob\Big(\liminf_{j\to\infty} E_{k,j}\Big) = 1\] It implies that for some large number $j_c$, $\Prob(E_{k,j}) = 1$, for all $j\geq j_c$. Therefore, for all finite $k>0$, there is \[\Prob\Big(\liminf_{j\to\infty} E_{k,j}\Big) = 1\]\telos

In fact, the framework of \sststar\ is rather flexible. By tuning the expression of $K(j)$, the guarantee can be as strong as \rrtstar\ at the cost of more computation. Consider a new version of Alg. \ref{alg:SSTstar} where switch line 6 to be \[K\leftarrow j\cdot\xi^{-(d+w+1)j}\cdot k_0\]

\begin{coro}
The version of \sststar\ where $K\leftarrow j\cdot\xi^{-(d+w+1)j}\cdot k_0$ guarantees to return a near-optimal trajectory in sufficiently large finite time, e.g. \[\mathbb{P}\Big(\liminf_{j\to\infty}E_{k,j}\Big)=1\]
\label{thm:SSTstarOverComplete}
\end{coro}

The proof is rather simple and very similar to the proof of Corollary \ref{coro:zeta}. The difference is that Eq. \ref{zeta} becomes 
\begin{align} \sum_{j=1}^\infty \Prob(\neg E_{k,j}) < P_c\cdot \sum_{j=1}^\infty (e^{-p_c\beta})^j \label{geometric}\end{align} It is a geometric series instead of \emph{Riemann zeta} function. For all possible $k_0 > 0$, Eq. \ref{geometric} converges. 


